Multi-task Learning for Real-time Autonomous Driving Leveraging Task-adaptive Attention Generator

Real-time processing is crucial in autonomous driving systems due to the imperative of instantaneous decision-making and rapid response. In real-world scenarios, autonomous vehicles are continuously tasked with interpreting their surroundings, analyzing intricate sensor data, and making decisions within split seconds to ensure safety through numerous computer vision tasks. In this paper, we present a new real-time multi-task network adept at three vital autonomous driving tasks: monocular 3D object detection, semantic segmentation, and dense depth estimation. To counter the challenge of negative transfer, which is the prevalent issue in multi-task learning, we introduce a task-adaptive attention generator. This generator is designed to automatically discern interrelations across the three tasks and arrange the task-sharing pattern, all while leveraging the efficiency of the hard-parameter sharing approach. To the best of our knowledge, the proposed model is pioneering in its capability to concurrently handle multiple tasks, notably 3D object detection, while maintaining real-time processing speeds. Our rigorously optimized network, when tested on the Cityscapes-3D datasets, consistently outperforms various baseline models. Moreover, an in-depth ablation study substantiates the efficacy of the methodologies integrated into our framework.

==> unused_materials.tex <==
\begin{comment}
1. 제안된 architecture는 TAG module의 유무와 상관없이 detection task에서 강세를 보인다. semantic segmentation의 경우, 비슷한 inference time을 가지는 ddr23에 비해 $-3.97\%p$의 성능하락을 보였지만, detection score에서 notable margin을 보였다.
2. Ours with TAG는 semantic segmentation metric을 제외한 모든 metric에서 증가된 성능을 보였고, averaged relative performance $\Delta \mathcal{T}$에서 유일하게 single-task setup보다 증가된 성능을 보임. second best인 DDR39에 비해 $+1.64\%p$ 증가된 성능과, 33.4\%의 inference time 감소를 보임.
3. DDRNet-39는 real-time이 아니고, Ours with TAG보다 약 1.5배의 inference time을 요구합니다.
\end{comment}
% \subsubsection{Evaluation results on VKITTI2}

% \subsection{Ablation stuidies}
% To validate the effectiveness of our proposed 



%the significance of task-generic spatial attention $\beta$ in directing the focus of the model towards spatial cues, resulting in a pronounced emphasis on object boundaries and smaller entities.
%, drawing attention to boundaries and small objects.

% \textcolor{red}{Please write one more sentence about the analysis (or role) of fig4-(b) results.}
% \end{comment}
% As shown in \figref{fig:attn}-(b), we observe that spatial attention %generally highlights (red) the salient objects and obstacles and mainly suppresses (blue) the drivable road and vegetation classes without direct supervision.
%Also, TAG seems to effectively extract the boundary of small objects in the image plane (e.g. pole groups, traffic signs), which are easily ignored in downsampled features from deep layers.
% Similar to the observation in~\cite{xu2023pidnet}, we believe that extracting spatial attention from the output of the high-resolution branch encourages the model to enhance the spatial details and alleviates the overshoot problem in object boundaries.

% These observation imply that our task-specific channel attention can 
% To demonstrate the effectiveness of channel attention in TAG, we organize an extensive experiment of task correlation across three tasks with respect to training iterations.
% As a metric of the task correlation, we follow the method of~\cite{sun2020adashare} that measures the cosine similarity among the attention sets, which are generated from the validation set of Cityscapes-3D.
% This metric effectively represents the correlation between tasks as it indicates which activated channels within channel attention are beneficial for each task.
% % ($\geq$ 20K iter)

% As depicted in \figref{fig:attn}, we observe that our TAG module can adaptively generate task-specific channel attention by localizing the task-specific channel position along the channel dimension of the semantic feature.
% We also found the three key-observation as follows:
% \begin{itemize}
%     \item[(1)] After the training, all correlations of task pairs have high values (0.84-0.90) because the proposed model capacity is restricted.
%     \item[(2)] The correlation depth estimation and 3D object detection is the most relative task pair due to the object depth estimation, which is the sub-task of 3D object detection, is closely related to depth estimation~\cite{park2021pseudo, wu2022attention, huang2022monodtr, chen2022pseudo, wang2019pseudo, ding2020learning, reading2021categorical}.
%     \item[(3)] Correlation between \{depth $\leftrightarrow$ 3D det.\} and \{depth $\leftrightarrow$ Seg.\} have higher value than \{3D det. $\leftrightarrow$ Seg.\}. This result indicates that the depth task serves as a bridge between semantic segmentation and the 3D detection task.
% \end{itemize}

% Additionally, we visualize the task-generic spatial attention to demonstrate which spatial areas in feature space are emphasized (or suppressed) by the TAG module.
% As shown in \figref{fig:attn}-(b), we observe that spatial attention generally highlights (blue) the salient objects and obstacles and mainly suppresses (red) the drivable road and vegetation classes without direct supervision.
% Also, TAG seems to effectively extract the boundary of small objects in the image plane (e.g. pole groups, traffic signs), which are easily ignored in downsampled features from deep layers.
% % Similar to the observation in~\cite{xu2023pidnet}, we believe that extracting spatial attention from the output of the high-resolution branch encourages the model to enhance the spatial details and alleviates the overshoot problem in object boundaries.
\begin{comment}
    5-1. 반면 soft-parameter sharing scheme의 computational cost 증가를 완화하기 위해 우리는 MTL에서 효율적으로 쓰이는 attention-based method를 이용해 적합한 task-wise feature를 생성하는 모듈인 Task-wise attention generator을 제안한다.
    5-2. dual pathway에서 semantic 정보를 가지고 있는 low-res branch에서 channel attention을, detail을 담당하는 high-res branch에서 spatial attention을 생성하여 task의 적합한 feature를 highlight/suppress 해주는 역할
\end{comment}
\begin{comment}
    6-1. In the evaluation results on two autonomous driving datasets; Cityscapes 3D and Virtual KITTI 2, our proposed model outperforms the existing baselines with notable margins.
    6-2. We conduct ablation studies of the proposed architecture and TAG module to validate the effectiveness of the proposed methods.
    6-3. Also, we report the extensive experiments that show how the TAG module effectively generates the task-specific feature by an attention-based mechanism.
    6-3. Our contributions are summarized as follows:
    \begin{itemize}
        \item We propose the first real-time autonomous driving framework capable of performing three crucial tasks: 3D object detection, semantic segmentation, and dense depth estimation.
        \item We propose the multi-task learning schemes that mitigate the negative transfer problem which is the ill-posed problem in multi-task learning while maintaining the model inference cost.
        \item Our framework achieves the best performance and efficiency compared to other baselines consisting of various backbones.
    \end{itemize}
\end{comment}

\begin{comment}
    To demonstrate the effectiveness of channel attention in TAG, we organize an extensive experiment of task correlation across three tasks with respect to training iterations.
    As a metric of the task correlation, We follow the method of~\cite{sun2020adashare} that measures the cosine similarity among the attention sets, which are generated from the validation set of Cityscapes-3D.
    This metric effectively represents the correlation between tasks as it indicates which activated channels within channel attention are beneficial for each task.
    We observe that  ($\geq$ 20K iter)
    1. Our TAG module can adaptively generate the task-adaptive channel attention by localizing the task-specific channel position from semantic feature
    After the 20000 iterations, the channel attention generator is saturated
    2. Model capacity가 적기 때문에 task correlation as cosine similarity가 높은 값을 유지함
    3. depth <-> 3ddet가 most-relative task pair, 이는 3D object detection의 sub-task인 object center depth task가 depth와 깊은 연관이 있는 것 때문~\cite{CMKD}
    4. depth <-> 3ddet, depth <-> seg가 det <-> seg에 비해 높은 cos-sim을 가지고 있다. depth가 det, seg를 bridging해주는 것으로 보인다. (본 논문에 별로 도움이 안될듯)
\end{comment}
% We found that the depth estimation task~~ (실험결과 뽑고 정리)
% In such scenarios, an applicable learning scheme is hard-parameter sharing (a.k.a. shared-bottom), which trains the multiple tasks within a single model.

% there is a risk of encountering the negative transfer problem, which leads to a decrease in performance among less-related tasks.
% However, it comes with the challenge of the negative transfer problem, where unrelated tasks may lead to a decrease in overall performance.
% This approach allows us to reduce the memory/time complexity of neural networks to nearly their lower bounds.

% This approach can effectively optimize the memory/time complexity of the network, but {negative transfer 설명}
% use the additional network layers or parameters
% These methods can mitigate the negative-transfer problem by using more loose constraints across tasks than hard-parameter sharing schemes, but 

% \begin{comment}
%     3-1. Hence, to design the real-time multi-task learning framework for autonomous driving, we adopt the hard-parameter sharing (a.k.a. shared-bottom)
%     3-2. 
%     3-2. how to mitigate the negative transfer problem?
%     우리는 memory/time complexity를 거의 lower bounds에 가깝게 할 수 있는 hard-parameter sharing 기반의 
% \end{comment}


% 자율주행을 위해서 다양한 perception tasks를 동시에 빠르고 정확하게 처리해야한다.
% 최근 딥러닝의 발전으로 monocular image로 부터 다양한 perception tasks 분야에서 뛰어난 성능을 가지는 single task 모델들이 연구되었다.
% 하지만 자율주행은 practical application이기 때문에 latency \& memory efficiency가 매우 중요하다.
% 따라서 task마다 개별적인 single network를 학습하는 것은 latency측면에서 매우 비효율적이다.
% 자율주행에서 필수적으로 필요한 Monocualr 3D object detection, Semantic segmentation, depth estimation을 포함하는 2D, 3D perception tasks를 하나의 모델로 통합하는 방법으로 Multi-task learning이 적합하다.
% 이전 Multi-task learning 연구에서 이러한 문제를 해결하려고 하였지만, 그대로 사용하기에는 layency 측면이 매우 부족하다.

% latency를 줄이기 위한 Multi-task learning 기법 중 하나는 hard-parameter sharing이다.
% Hard-parameter sharing~\cite{} is the method, which is training the shared front-end of the network with multiple tasks while training specific classifiers for each task to obtain the outputs as different modalities.
% This approach allows us to reduce the memory/time complexity of neural networks to nearly their lower bounds.
% However, it comes with the challenge of the negative transfer problem, where unrelated tasks may lead to a decrease in overall performance.
% 또한, 각 태스크 별로 성능 향상을 위해 필요로 하는 feature가 다르다. 예를 들어, 3D object detection은 더 뛰어난 성능을 위해 multi-scale feature가 필요로 하고, Semantic segmentation은 high-resolution feature의 detail을 필요로 한다.

% 이러한 문제를 해결하기 위해 하드파라미터 쉐어링을 사용하는 네트워크 구조 개발 ?

% Autonomous Driving is now at the forefront of transportation technology.
% One of the fundamental challenges in achieving a fully autonomous driving system for vehicles lies in endowing them with the ability to multi-task including 3D object detection, semantic segmentation, and depth estimation.
% Training the single networks for each task is notably inefficient in autonomous driving, considering the essential factors of memory efficiency and latency in practical autonomous driving systems.
% For this reason, many autonomous driving modules adopt the multi-task learning method, which is the method that trains multiple tasks to a single network, to optimize the computational cost of deep learning networks.

% Multi-task learning can be broadly categorized into two main approaches: hard-parameter sharing~\cite{} (\textit{a.k.a} shared-bottom) and soft-parameter sharing~\cite{}.
% Hard-parameter sharing~\cite{} is the method, which is training the shared front-end of the network with multiple tasks while training specific classifiers for each task to obtain the outputs as different modalities.
% This approach allows us to reduce the memory/time complexity of neural networks to nearly their lower bounds.
% However, it comes with the challenge of the negative transfer problem, where unrelated tasks may lead to a decrease in overall performance.
% % This approach can effectively optimize the memory/time complexity of the network, but {negative transfer 설명}
% Unlike hard-parameter sharing, where layers are explicitly shared across tasks, soft-parameter sharing~\cite{} allows the model to have separate sets of parameters while encouraging some level of parameter similarity or correlation across tasks.
% These approaches are particularly useful, as they can mitigate the risk of the negative transfer problem that can occur with hard-parameter sharing.
% However, Most of these methods use additional network layers or parameters in proportion to the number of tasks, making the time/memory complexity almost equivalent to training multiple single-task models.
% % use the additional network layers or parameters
% % These methods can mitigate the negative-transfer problem by using more loose constraints across tasks than hard-parameter sharing schemes, but 

% More recent works~\cite{adashare, den, controllable, LTB, dynamic neural...} have been proposed to dynamically control the ratio of shared parameters across tasks using Nas-style methods to construct a task adaptive sub-network.
% These methods achieve outperforming accuracyWithin this trade-off between the computational efficiency and accuracy of the model, We attempt to strike a balance between leveraging shared knowledge across tasks and allowing flexibility for task-specific learning while gaining the computational efficiency of hard-parameter sharing schemes.
% Inspired by multi-resolution networks for real-time segmentation~\cite{ddrnet, icnet, pidnet}, We present a novel real-time multi-task network architecture capable of performing three crucial tasks in autonomous driving: 3D object detection, semantic segmentation, and dense depth estimation.
% To mitigate the negative transfer, We propose the {method name} that can automatically find the task relations across three tasks and arrange the task-sharing pattern while gaining the efficiency of the hard-parameter sharing method.
% We also propose the utilize loss that encourages each task-specific attention to utilize the most channel with high capacity while searching the optimal task-sharing pattern, concurrently.
% To the best of our knowledge, our model is the first model that is capable of performing multiple tasks, including 3D object detection, while ensuring real-time algorithmic speed.

% % We propose the {method name} that shared-bottom의 computational efficiency를 유지하되, 태스크 간의 negative-trasnfer를 완화하기 위해 network의 sharing pattern을 channel attention-based method로 학습하는.
% % Also, We propose the {method: i.e. modality translation} {method 설명}
% % This method can not only mitigate the negative transfer problem by considering the task relation through the attention mechanism but also maintain the inference time.

% In the evaluation results on two autonomous driving datasets; Cityscapes 3D and Virtual KITTI 2, our proposed model outperforms the existing baselines with notable margins.
% Our contributions are summarized as follows:
% \begin{itemize}
%     \item We propose the first real-time autonomous driving framework capable of performing three crucial tasks: 3D object detection, semantic segmentation, and dense depth estimation.
%     \item We propose the multi-task learning schemes that mitigate the negative transfer problem which is the ill-posed problem in multi-task learning while maintaining the model inference cost.
%     \item Our framework achieves the best performance and efficiency compared to other baselines consisting of various backbones.
% \end{itemize}


% % propose the real-time multi-task learning network architecture for autonomous driving 
% % Within these trade-off between model efficiency and accuracy, the model should achieve a certain lev
% % 이 문제를 해결하기 위해서는 여러 태스크를 한개의 네트워크에서 학습하는 Multi-task learning 기법을 사용해야 한다.

% \begin{comment}
    
%     % Inspired by real-time semantic segmentation~\cite{ddr, bisenet, ...} and monocular 3D object detection~\cite{monodle, monocon, ...} we emerge the flagship architectures of each field.
%     % 4-3. semantic segmentation에서의 design  by automatically learning the task-wise sharing patterns (\textit{i.e.} determining which layers in the network should be shared across which tasks.), but these also share the scalability issues that soft-parameter sharing methods have.

% contribution
% Within this trade-off between the computational efficiency and accuracy of the model, We attempt to strike a balance between leveraging shared knowledge across tasks and allowing flexibility for task-specific learning while gaining the computational efficiency of hard-parameter sharing schemes.
% Inspired by multi-resolution networks for real-time segmentation~\cite{ddrnet, icnet, pidnet}, We present a novel real-time multi-task network architecture capable of performing three crucial tasks in autonomous driving: 3D object detection, semantic segmentation, and dense depth estimation.
% To mitigate the negative transfer, We propose the {method name} that can automatically find the task relations across three tasks and arrange the task-sharing pattern while gaining the efficiency of the hard-parameter sharing method.
% We also propose the utilize loss that encourages each task-specific attention to utilize the most channel with high capacity while searching the optimal task-sharing pattern, concurrently.
% To the best of our knowledge, our model is the first model that is capable of performing multiple tasks, including 3D object detection, while ensuring real-time algorithmic speed.

% % We propose the {method name} that shared-bottom의 computational efficiency를 유지하되, 태스크 간의 negative-trasnfer를 완화하기 위해 network의 sharing pattern을 channel attention-based method로 학습하는.
% % Also, We propose the {method: i.e. modality translation} {method 설명}
% % This method can not only mitigate the negative transfer problem by considering the task relation through the attention mechanism but also maintain the inference time.

% In the evaluation results on two autonomous driving datasets; Cityscapes 3D and Virtual KITTI 2, our proposed model outperforms the existing baselines with notable margins.
% Our contributions are summarized as follows:
% \begin{itemize}
%     \item We propose the first real-time autonomous driving framework capable of performing three crucial tasks: 3D object detection, semantic segmentation, and dense depth estimation.
%     \item We propose the multi-task learning schemes that mitigate the negative transfer problem which is the ill-posed problem in multi-task learning while maintaining the model inference cost.
%     \item Our framework achieves the best performance and efficiency compared to other baselines consisting of various backbones.
% \end{itemize}


% % propose the real-time multi-task learning network architecture for autonomous driving 
% % Within these trade-off between model efficiency and accuracy, the model should achieve a certain lev
% % 이 문제를 해결하기 위해서는 여러 태스크를 한개의 네트워크에서 학습하는 Multi-task learning 기법을 사용해야 한다.

% \begin{comment}
    
%     % Inspired by real-time semantic segmentation~\cite{ddr, bisenet, ...} and monocular 3D object detection~\cite{monodle, monocon, ...} we emerge the flagship architectures of each field.
%     % 4-3. semantic segmentation에서의 design 
    
    
%     Attention-based method~\cite{MTAN, ATTNMT} 를 사용하여 task 마다 적합한 task-wise feature를 도출하여 negative transfer를 완화할 수 있는 deep learning framework를 제안한다.
    


%     * 우리는 autonomous driving에 필요한 perception task를 hard-parameter sharing 기법으로 효율적으로 학습할 수 있는 real-time multi-task learning을 위해서 새로운 deep learning architecture를 설계하였다.
%     * real-time semantic segementation, real-time object detection 의 design에 영감을 받아, dual-pathway, feature aggregation으로 object detection과, semantic segmentation, dense-depth estimation을 모두 효율적으로 처리할 수 있다.
%     ** 또한 hard-parameter sharing scheme의 algorithmic efficiency를 최대한 보존하면서, negative transfer를 완화할 수 있는 attention-based MTL schemes를 개발하였다.
%     ** MTAN, other attention-based MTL에서 attention-based method가 conditional computation에 영향을 줄 수 있다는 점에서 기인하여, 연산량을 거의 증가시키지 않고 task에 적합한 feature를 도출해내는 방법.
%     ** semantic 정보를 뽑아내는 low-res pathway에서 channel attention을, detail을 책임지는 high-res pathway에서 task-wise spatial attention을 추출
%     *** monocular 3D object detection을 포함한 real-time multi-task learning 비교군이 없기때문에 우리는 real-time을 목적으로 한 다양한 single network architecture의 backbone과 제안된 architecture를 비교 (4.experiment section으로 가라)
%     *** 


% \end{comment}

% This approach allows us to reduce the memory/time complexity of neural networks to nearly their lower bounds and also can improve the generalization ability by consolidating information from various related tasks into a joint feature space.

% \begin{comment}
%     3-1. MTAN, adashare, Dynamic~ 등의 other soft-parameter sharing scheme들은 직접적으로 parameter를 공유하는 것보다 약한 restriction (L2-regulerization, conditional computation, attention, etc.) 를 사용하여 negative transfer를 완화하였지만, hard-parameter sharing scheme의 computational cost에서의 이점을 그대로 가져오지 못했다는 단점이 존재한다.
%     3-2. 이러한 trade-off 안에서 우리는 real-time framework를 위해서 우리는 hard-parameter sharing scheme의 computational efficiency를 보존하는 반면, 자율주행 태스크에 필요한 crucial task의 negative transfer를 완화하는 방법을 찾아야 한다.
%     3-3. 이 목표를 달성하기 위해서 우리는 두가지의 key-component를 고려하였다: 1. feasible multi-task architecture for autonomous driving, 2. MTL schemes to generate the task-wise features
% \end{comment}
% Unlike hard-parameter sharing, where layers are explicitly shared across tasks, soft-parameter sharing~\cite{} and Nas-style MTL allow the model to have separate sets of parameters while encouraging some level of parameter similarity or correlation across tasks.

% Within this trade-off between the computational efficiency and accuracy of the model, We attempt to strike a balance between leveraging shared knowledge across tasks and allowing flexibility for task-specific learning while gaining the computational efficiency of hard-parameter sharing schemes.
% We consider two components to achieve this objective; 

% Inspired by multi-resolution networks for real-time segmentation~\cite{ddrnet, icnet, pidnet}, We present a novel real-time multi-task network architecture capable of performing three crucial tasks in autonomous driving: 3D object detection, semantic segmentation, and dense depth estimation.
% To mitigate the negative transfer, We propose the {method name} that can automatically find the task relations across three tasks and arrange the task-sharing pattern while gaining the efficiency of the hard-parameter sharing method.
% We also propose the utilize loss that encourages each task-specific attention to utilize the most channel with high capacity while searching the optimal task-sharing pattern, concurrently.
% To the best of our knowledge, our model is the first model that is capable of performing multiple tasks, including 3D object detection, while ensuring real-time algorithmic speed.

% per-pixel regression task인 semantic segementation과 dense depth estimation을 efficient and effective하게 수행할 수 있는 two-pathway architecture를 기반으로 다양한 객체의 크기를 탐지하는데 도움이 되는 feature aggregation
% two-pathway architecture
% 의 crucial architectural element가 다르기 때문에, 우리는 두 가공방법의 key-component를 가져와서 hybrid 형태의 backbone을 design하였다.

% 각 태스크들의 crucial architectural design 방식이 다르기 때문에 우리는 

% Inspired by multi-resolution networks for real-time segmentation~\cite{ddrnet, icnet, pidnet}, We present a novel real-time multi-task network architecture capable of performing three crucial tasks in autonomous driving: 3D object detection, semantic segmentation, and dense depth estimation.

\begin{comment}
    4-1. {Multi-task architecture} we first choose the crucial tasks of autonomous driving as follows: 3D object detection, semantic segmentation, and dense depth estimation.
    4-2. object detection에서는 다양한 크기를 가진 객체를 추정해야 하기 때문에 높은 성능을 위해서 다양한 receptive field를 가진 intermediate feature를 aggregate하는 모델~\cite{monocon, monodle, 등등} 이 높은 성능을 보이고 있다.
    4-3. On the other hand, semantic segementation에서는 HRNet에 기반하여 low-resolution의 semantic information과 hig-resolution의 detail을 각각 담당하는 two-pathway architecture가 best trade-of curve를 보여주고 있다.
    4-4. 따라서 우리는 이러한 모델의 구조를 hybrid 형태로 합친 모델 architecture를 제안한다.
\end{comment}
